Malicious Network Traffic Detection via Deep Learning: An Information Theoretic View

The attention that deep learning has garnered from the academic community and industry continues to grow year over year, and it has been said that we are in a new golden age of artificial intelligence research. However, neural networks are still often seen as a "black box" where learning occurs but cannot be understood in a human-interpretable way. Since these machine learning systems are increasingly being adopted in security contexts, it is important to explore these interpretations. We consider an Android malware traffic dataset for approaching this problem. Then, using the information plane, we explore how homeomorphism affects learned representation of the data and the invariance of the mutual information captured by the parameters on that data. We empirically validate these results, using accuracy as a second measure of similarity of learned representations. Our results suggest that although the details of learned representations and the specific coordinate system defined over the manifold of all parameters differ slightly, the functional approximations are the same. Furthermore, our results show that since mutual information remains invariant under homeomorphism, only feature engineering methods that alter the entropy of the dataset will change the outcome of the neural network. This means that for some datasets and tasks, neural networks require meaningful, human-driven feature engineering or changes in architecture to provide enough information for the neural network to generate a sufficient statistic. Applying our results can serve to guide analysis methods for machine learning engineers and suggests that neural networks that can exploit the convolution theorem are equally accurate as standard convolutional neural networks, and can be more computationally efficient.

==> text/05-dedication.tex <==
% Adds a spacer where the header would be
\chapter*{~}
\addcontentsline{toc}{chapter}{Dedication}

\begin{center}
\textit{Dedicated to Courtney, my loving wife\\
and mother of my three wretched boyes.\\
I could not do this without you.\\[36pt]}
\end{center}

==> text/15-my-original-cv.tex <==
% Add to TOC
\addcontentsline{toc}{chapter}{Curriculum vitae}

% If you want to remove page numbers
%\pagestyle{empty}


% Default settings for enumerate environment
\setenumerate{wide=0em,%
              leftmargin=*,
              labelindent=0pt,
              label=\textbullet,
              noitemsep,
              topsep=0pt,
              parsep=0pt,
              before=\rmfamily}

% Remove indentation
\setlength{\parindent}{0pt}

% Space between paragraphs
\setlength{\parskip}{6pt}

% No added spaces after periods
\frenchspacing

% For a reasonable fit
\footnotesize

\textbf{\small Curriculum Vitae\hfill\large Erick Galinkin\hfill\small June, 2020}
\begin{center}
(+1) 631.830.7524\\
{\color{blue} \ul{\sffamily\textit{egalink1@jhu.edu}}}
\end{center}

% change font 
\sffamily

\textbf{EDUCATION AND DEGREES}

\ul{2018--Present} Graduate student,
Department of Applied and Computational Mathematics\\
Johns Hopkins University

\ul{20XX--20XX} Undergraduate student,
Department of Biology
University of California


\textbf{RESEARCH EXPERIENCE}

\textit{Johns Hopkins University, Some specific school}\\
\textit{Department of Biology\hfill(MONTH YEAR-Present)}\\
\textbf{\rmfamily Graduate Student in the laboratory of a \ul{Principal Investigator}}

\begin{enumerate}
\item Some thing I did.
\item Another thing I did.
\item Yet another thing I did.
\end{enumerate}

\textit{A previous academic research institution, LOCATION\hfill(MONTH YEAR-MONTH YEAR)}\\
\textbf{\rmfamily Post-baccalaureate Researcher in the laboratory of a \ul{Principal Investigator}}

\begin{enumerate}
\item A thing I did.
\item Another thing I did.
\end{enumerate}

\textit{A previous academic research institution, LOCATION\hfill(MONTH YEAR-MONTH YEAR)}\\
\textbf{\rmfamily A previous position in the laboratory of a \ul{Principal Investigator}}

\begin{enumerate}
\item Some thing I did.
\item Another thing I did.
\item Yet another thing I did.
\end{enumerate}

\textbf{TECHNIQUES AND SKILLS}

\textbf{\rmfamily Molecular Techniques}

\textrm{\noindent DNA/RNA/Protein extraction and purification ; PCR ; RT-PCR ; Quantitative 
PCR ; DNA Sequence Analysis ; Southern Blot ; Western Blot ; SDS-PAGE ; Ultra-Centrifugation 
; Agarose Gel Electrophoresis/Imaging ; \textit{Drosophila} Microinjection ;\textit{ 
Anopheles} Microinjection ; Fluorescence Microscopy ; Immunofluorescence Microscopy ; 
Cell/tissue Culture ; Cell Transfection ; Antiseptic Technique}

\textbf{\rmfamily Computing and Other Skills}
\begin{enumerate}
\item Power user of both Windows and Macintosh platform software and hardware
\item Basic user of Linux/Unix systems
\item Basic Perl programming
\item Basic R programming
\item Proper waste disposal practices and safety training
\item Radioactive isotope certification and safety training
\item Ethical use of vertebrate animals (mice) in research training
\end{enumerate}

\textbf{TEACHING EXPERIENCE}

\textit{Johns Hopkins University, Some school\hfill(MONTH YEAR-MONTH YEAR)}\\
\textbf{\rmfamily Teaching Assistant}
\begin{enumerate}
\item Graduate Student Instructor for a class
\end{enumerate}

\textit{University of California\hfill(MONTH YEAR-MONTH YEAR)}\\
\textbf{\rmfamily Teaching Assistant}
\begin{enumerate}
\item Undergraduate Student Instructor for a class.
\end{enumerate}


\textbf{PUBLICATIONS}

% change font back to roman
\rmfamily

{\color{blue} \ul{The title of my article.}} 
A. Anderson, \textbf{Myself}, B. Baldwin, C. Cortez and 
D. Dylan. \textit{Journal Name} \textbf{VOLUME}. PAGES (YEAR).

{\color{blue} \ul{The title of my article.}} 
A. Anderson, \textbf{Myself}, B. Baldwin, C. Cortez and 
D. Dylan. \textit{Journal Name} \textbf{VOLUME}. PAGES (YEAR).

{\color{blue} \ul{The title of my article.}} 
A. Anderson, \textbf{Myself}, B. Baldwin, C. Cortez and 
D. Dylan. \textit{Journal Name} \textbf{VOLUME}. PAGES (YEAR).

{\color{blue} \ul{The title of my article.}} 
A. Anderson, \textbf{Myself}, B. Baldwin, C. Cortez and 
D. Dylan. \textit{Journal Name} \textbf{VOLUME}. PAGES (YEAR).

{\color{blue} \ul{The title of my article.}} 
A. Anderson, \textbf{Myself}, B. Baldwin, C. Cortez and 
D. Dylan. \textit{Journal Name} \textbf{VOLUME}. PAGES (YEAR).

